RETSim: Resilient and Efficient Text Similarity

This paper introduces RETSim (Resilient and Efficient Text Similarity), a lightweight, multilingual deep learning model trained to produce robust metric embeddings for near-duplicate text retrieval, clustering, and dataset deduplication tasks. We demonstrate that RETSim is significantly more robust and accurate than MinHash and neural text embeddings, achieving new state-of-the-art performance on dataset deduplication, adversarial text retrieval benchmarks, and spam clustering tasks. We also introduce the W4NT3D benchmark (Wiki-40B 4dversarial Near-T3xt Dataset) for evaluating multilingual, near-duplicate text retrieval capabilities under adversarial settings. RETSim and the W4NT3D benchmark are open-sourced under the MIT License at https://github.com/google/unisim.

==> acknowledgements.tex <==
\label{sec:ack}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

==> real_world_dedup.tex <==
\subsection{CORE Near-Duplicates Dataset Evaluation}
\label{sec:neardup}

We benchmark on two real-world near-duplication detection datasets, NEWS-COPY and scholarly articles

\subsubsection{Setup}

\paragraph{Scholarly Articles Dataset}

\begin{table}[ht]
\centering
\scalebox{0.83}{\begin{tabular}{@{}l|cccccc@{}}
\toprule
 \multirow{2}{*}{\textbf{Model / Algorithm}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}c@{}}Precision \\ Duplicates\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}c@{}}Recall \\ Duplicates\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}c@{}}Precision \\ Non-Duplicates\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}c@{}}Precision \\ Non-Duplicates\end{tabular}}} & \multicolumn{1}{l}{\textbf{Macro F1}} & \multicolumn{1}{l}{\textbf{Accuracy}} \\ \midrule
Exact Title Matching* & 0.830 & 0.50 & 0.709 & \textbf{0.992} & 0.757 & 0.746 \\
Hybrid Method* & 0.908 & 0.83 & 0.899 & \underline{0.979} & 0.904 & 0.903 \\
SimHash LSH & 0.869 & 0.669 & 0.761 & 0.913 & 0.793 & 0.791 \\
MinHash LSH & \underline{0.929} & 0.902 & 0.915 & 0.938 & 0.921 & 0.918 \\   \midrule
\rpd & \textbf{0.945} & \textbf{0.941} & \textbf{0.945} & 0.949 & \textbf{0.945} & \textbf{0.928} \\
\rnd & 0.928 & \underline{0.937} & \underline{0.942} & 0.934 & \underline{0.935} & \underline{0.926} \\ \bottomrule
\end{tabular}}
\caption{\fixme results on scholarly articles dedup dataset}
\label{tab:scholar}
\end{table}

\paragraph{NEWS-COPY Dataset}

% \begin{figure}
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.4\linewidth]{figures/partial_dup_threshold.png}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.5\linewidth]{figures/near_dup_threshold.png}
% \end{subfigure}
% \caption{Thresholds}
% \label{fig:dedup_threshold}
% \end{figure}



\begin{table}[ht]
\begin{minipage}[b]{0.45\linewidth}
\centering
\begin{tabular}{@{}l|rl@{}}
\toprule
% \multicolumn{1}{c}{\textbf{Model/Algorithm}} & \multicolumn{1}{l}{\textbf{ARI}} &  \\ \midrule
\multicolumn{1}{c|}{\textbf{Model/Algorithm}} & \multicolumn{1}{l}{\textbf{ARI}} &  \\ \midrule
Multilingual USE & 0.730 &  \\
Multilingual E5-Base & 0.742 &  \\
S-BERT* & 0.700 &  \\ 
 \midrule
SimHash & 0.695 &  \\
MinHash* & 0.737 &  \\
MinHash (Ours) & \underline{0.783} &  \\ 
 \midrule
\rpd & \textbf{0.831} &  \\
\rnd & 0.704 &  \\ \bottomrule
\end{tabular}
    \caption{\fixme Adjusted Rand Index (ARI) on NEWS-COPY dataset. * denotes results reported in \citep{}.}
    \label{tab:news_copy_ari}
\end{minipage}\hfill
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/news_copy_dedup_length.pdf}
\vspace{-0.8cm}
\captionof{figure}{\fixme  news copy dataset by longer text divided by shorter text in a dup pair. this is a longer caption ha}
\label{fig:length_ratio_news_copy}
\end{minipage}
\end{table}


% \begin{table}[h]
% \begin{tabular}{@{}l|rl@{}}
% \toprule
% % \multicolumn{1}{c}{\textbf{Model/Algorithm}} & \multicolumn{1}{l}{\textbf{ARI}} &  \\ \midrule
% \multicolumn{1}{c|}{\textbf{Model/Algorithm}} & \multicolumn{1}{l}{\textbf{ARI}} &  \\ \midrule
% Multilingual USE & 0.730 &  \\
% Multilingual E5-Base & 0.742 &  \\
% S-BERT* & 0.700 &  \\
% MinHash* & 0.737 &  \\
% MinHash (Ours) & \underline{0.783} &  \\
% SimHash & 0.695 &  \\
% \rpd & \textbf{0.831} &  \\
% \rnd & 0.704 &  \\ \bottomrule
% \end{tabular}
%     \caption{\fixme  n }%
%     \label{fig:news_copy_ari}%
% \end{table}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.6\textwidth]{figures/news_copy_dedup_length.pdf}
% \caption{\fixme  news copy dataset by longer text divided by shorter text in a dup pair }
% \label{fig:length_ratio_news_copy}
% \end{figure}



==> refs.tex <==
\section{References}
\label{sec:ref}

\bibliographystyle{ACM-Reference-Format} 
\bibliography{refs}

==> textyard.tex <==
One of the main challenges in comparing clustering performance is to have accurately labeled ground truth data for spam campaigns. This is labor intensive and hence not easy to come by. I resorted to using several heuristics to generate this data:

\begin{enumerate}
    \item Using the first 5 words of the subject as the campaign identifier for ground truth labels. One of the main concerns here is that this would lead to overclustering. In general this might be true; if we consider all emails, the subject of a spam email could be similar to the subject of a benign one. However, here we only consider those emails which have been reported as spam by trusted users. The volume of these emails is much smaller (since we have already filtered out obviously benign emails) and using the first 5 words of the subject is a good heuristic.
    \item Some users might report emails that are not actually spam as spam due to ambiguity on the meaning of spam. The most common example of this is promotional emails. Examples include emails from zillow of the form “10 homes we think you'll love” or from instagram of the form “new login to instagram from”. In these cases the SERP score of either the dk domain or the spf domain is very high and so we can again filter these out. However, I have intentionally included them as it gives us a good mix of objective spam and soft spam /benign campaigns. Additionally using the heuristic of the first 5 subject words works well for these too.
    \item Some spammers particularly the ones who use the “.*onmicrosoft.com” domains spread their spam campaigns over several domains, subjects etc. Since I mostly saw this only in the onmicrosoft domains I manually corrected for this [in the colab].
\end{enumerate}

I then created two datasets: one over which simhash seems to work well for clustering (GOOD DATASET) and one over which simhash seems to have very poor clustering performance (BAD DATASET). These were created by looking at the ratio of the number of simhashes / total number of messages for each potential spam campaign (based on the method above). The main idea here is that if the number of simhashes is almost equal to the number of messages then simhash has not been very good at clustering these messages. Hence for the GOOD DATASET we want campaigns with a low value of this ratio and for the BAD DATASET we want campaigns with a high value of this ratio. 

\subsubsection{Clustering Methods}

To compare simhash vs retsim we would need to decide on a clustering algorithm to use. Scikit learn offers a number of options here. Some factors that governed this choice.

\begin{enumerate}
    \item We would need an algorithm that supports non euclidean distances. Retsim uses the cosine distance and simhash uses the hamming distance, both of which are non euclidean. 
    \item We would like an algorithm that scales so that we can run it on larger datasets (size 1k - 5K).
    \item We easily have access to the number of clusters. Any algorithm which uses the number of clusters as the only parameter, makes parameter tuning much easier than say an algorithm which uses the inter cluster distance or some other parameter.
    \item The clusters are not very dense and can be small. Hence a density based clustering algorithm like dbscan might filter away some samples as noise.
\end{enumerate}

Given these considerations Agglomerative clustering seems to work best.

To evaluate the clustering performance we will use the following metrics:

\begin{enumerate}
    \item \textbf{homogeneity}: each cluster contains only members of a single class.
    \item \textbf{completeness}: all members of a given class are assigned to the same cluster.
    \item \textbf{V-measure (Normalized Mutual Information)}: Harmonic means of homogeneity and completeness
    \item \textbf{Adjusted Rand Index}: The Rand Index computes a similarity measure between two clusterings by considering all pairs of samples and counting pairs that are assigned in the same or different clusters in the predicted and true clusterings 
    \begin{center}
          $RI = \frac{\mbox{number of agreeing pairs}}{\mbox{number of pairs}}$  
    \end{center}

    \item \textbf{Silhouette Score}: This is a property of the clustering itself and does not need the ground truth values at all. It is a measure of the ratio between the intra-cluster distance to the inter cluster distance. A clustering which shows good inter and intra-cluster separation will have a value closer to 1. $a = $ The mean distance between a sample and all other points in the same class, and 
    $b = $ The mean distance between a sample and all other points in the next nearest cluster
    \begin{center}
      $ss = \frac{b-a}{max(b, a)}$      
    \end{center}
\end{enumerate}

The main reason for choosing these metrics was as follows:
\begin{enumerate}
    \item Homogeneity and completeness are simple and intuitive that help understand the clustering in general.
    \item V-measure helps to correct for the case where either homogeneity or completeness is much better at the expense of the other.
    \item Adjusted Rand Index helps to see how the clustering performs compared to a randomized clustering algorithm. Both homogeneity and completeness can be deceptively high for just a randomized clustering specially when the number of samples is not too high and the number of clusters is fairly high.
    \item Silhouette Score was chosen since it does not depend on the value of the true labels and entirely on the clustering itself.
\end{enumerate}



====


as reported in the benchmark section of our paper. However, we argue that this compromise is beneficial in practice as most text search and corpus de-duplication applications operate at the syntactic level, making \rs an ideal solution for these use-cases.




Our extensive benchmarks demonstrate that \rs performs competitively in retrieval tasks across multiple languages and significantly outperforms other algorithms in the presence of typos in the text and queries. -- something about nearduplciat\textbf{}




Finally, our evaluation results demonstrate that \rs excels in real-world text @anonymous applications, such as de-duplicating content at scale and powering active learning pipelines.



\note{TODO: Include goals and non-goals. Inference speed (cpu, gpu, and tpu) and model size}
\note{TODO: outline the expected use cases}




\subsection{Mixed dataset}
To ensure the model works consistently well across various languages and modalities, we use an evaluation dataset that combines examples from XL-Sum, Wiki-40B, The Stack (Smol)~\cite{kocetkov_stack_2022}. For each language in each dataset, we randomly select 500 target examples to index and 100 query examples which are selected from the aforementioned target examples. This yields a dataset with 49k indexed target examples and 9.8k queries.





We select the query size and target size from the cross product of the two sets $Q = \{8, 16, 32, 64, 128, 256. 512\}$ and $T= \{ 32, 64, 128, 256, 512 \}$, representing the query and target lengths respectively. For each of the settings, we have $10,000$ queries and $10,000$ targets of the selected size pairs p, $p \in Q \times T$. We design the queries and targets such that the shorter text is contained within the longer text. Let's assume that the selected size pair $p =(128,32)$, the query size is $128$ and the target size is $32$. we make sure that the target of length $32$ is contained within the query of length $128$. Similarly, if the query size is smaller than the target size, we make sure that the query is contained with the target. The dataset consists of 10,000 query, and 10,000 target texts for each of the 35 query and target size setting (cross product of $|Q| = 5$ and $|T| = 7$, $|Q \times T|= 35$). For the second task we further apply augmentation  to the queries. We have two types of augmentation, character and word level augmentations. Character level augmentations consist of character insertion, character deletion, character swap, and character substitution. Similarly word level augmentations consist of word insertion, word deletion, word swap and word substitution. Given a query we select a random location to perform the augmentation. The subset of the characters to be inserted, substituted with are selected from the alphabets of each languages. We do not perform cross lingual character augmentation. Similarly the words that are to be inserted or substituted with are selected from a bag of words that is created by using the samples from the corresponding language. We perform different percentages of augmentation, $20\%, 30\%, 40\%, 50\%, 60\%$ and $80\%$ for each of the character and word level augmentations. 


===

